Understanding multi-layered transmission matrices

Transmission matrices, mapping the propagation of light from one end of the tissue to the other, form an important mathematical tool in the analysis of tissue scattering and the design of wavefront shaping systems. To understand the relationship between their content and the volumetric structure of the tissue, we wish to fit them with multi-slice models, composed of a set of planar aberrations spaced throughout the volume. The number of layers used in such a model would largely affect the amount of information compression and the ease in which we can use such layered models in a wavefront-shaping system. This work offers a theoretical study of such multi-layered models. We attempt to understand how many layers are required for a good fit, and how does the approximation degrade when a smaller number of such layers is used. We show analytically that transmission matrices can be well fitted with very sparse layers. This leads to optimistic predictions on our ability to use them to design future wavefront shaping systems which can correct tissue aberration over a wide field-of-view.

==> cvpr_sec_files_cr/fig_fit_allMats.tex <==
\begin{figure*}[t!]
	\begin{center}
		\begin{tabular}{@{}c@{~~~~~~~}c@{}}	
			\begin{tabular}{@{}c@{~~~~}c@{}c@{}}	
			{\raisebox{1.90cm}{\rotatebox[origin=c]{90}{Monte Carlo }}}&
			\includegraphics[height=0.21\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51.pdf}&
			\includegraphics[height=0.21\textwidth]{figs/fitting_chen_mats/fit_chensmats_zmax51_corr.pdf}
				\end{tabular}&
				\begin{tabular}{@{}c@{}c@{}c@{}@{}c@{}c@{}c@{}}	
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum0}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum0_colorbar}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum1}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum1_colorbar}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum2}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum2_colorbar}\vspace{-0.2cm}\\
				$M=0$&&$M=1$&&$M=2$&\\
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum5}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum5_colorbar}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum10}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum10_colorbar}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum20}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_chen_mats/fit_chensmats_z_max51_OD5_layerNum20_colorbar}\vspace{-0.2cm}\\
				$M=5$&&$M=10$&&$M=20$&
				\end{tabular}\\
%				\begin{tabular}{@{}c@{~~~~}c@{}c@{}}		{\raisebox{1.90cm}{\rotatebox[origin=c]{90}{Chicken breast }}}&
%				\includegraphics[height=0.21\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_errplot.pdf}&
%				\includegraphics[height=0.21\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_corplot.pdf}
%			\end{tabular}&
%			\begin{tabular}{@{}c@{}c@{}c@{}@{}c@{}c@{}c@{}}	
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum0}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum0_colorbar}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum1}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum1_colorbar}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum2}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum2_colorbar}\vspace{-0.2cm}\\
%				$M=0$&&$M=1$&&$M=2$&\\
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum5}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum5_colorbar}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum10}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum10_colorbar}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum20}&
%				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_chicken/marina05_30_mats_z_max140_focusing_layerNum20_colorbar}\vspace{-0.2cm}\\
%				$M=5$&&$M=10$&&$M=20$&\\
%			\end{tabular}\\
				\begin{tabular}{@{}c@{~~~~}c@{}c@{}}	
				{\raisebox{1.90cm}{\rotatebox[origin=c]{90}{Parafilm }}}&
				\includegraphics[height=0.21\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_errplot.pdf}&
				\includegraphics[height=0.21\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_corplot.pdf}
			\end{tabular}&
			\begin{tabular}{@{}c@{}c@{}c@{}@{}c@{}c@{}c@{}}	
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum0}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum0_colorbar}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum1}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum1_colorbar}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum2}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum2_colorbar}\vspace{-0.2cm}\\
				$M=0$&&$M=1$&&$M=2$&\\
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum5}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum5_colorbar}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum10}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum10_colorbar}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum20}&
				\includegraphics[height=0.08\textwidth]{figs/fitting_marina_parafilm/marina05_26_mats_z_max35_focusing_layerNum20_colorbar}\vspace{-0.2cm}\\
				$M=5$&&$M=10$&&$M=20$&\\	
			\end{tabular}
		\\
			\begin{tabular}{@{}c@{~~~~}c@{}c@{}}	
			{\raisebox{1.90cm}{\rotatebox[origin=c]{90}{Brain}}}&
			\includegraphics[height=0.21\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_errplot.pdf}&
			\includegraphics[height=0.21\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_corplot.pdf}\\
			&	(a) Fitting error&(b) Delivered Eng.
		\end{tabular}&
		\begin{tabular}{@{}c@{}c@{}c@{}@{}c@{}c@{}c@{}}	
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum0}&
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum0_colorbar}&
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum1}&
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum1_colorbar}&
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum2}&
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum2_colorbar}\vspace{-0.2cm}\\
			$M=0$&&$M=1$&&$M=2$&\\
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum5}&
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum5_colorbar}&
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum10}&
			\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum10_colorbar}&&
			%\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum20}&
			%\includegraphics[height=0.08\textwidth]{figs/fitting_marina_brain/marina06_27_mats_z_max300_focusing_layerNum20_colorbar}\vspace{-0.2cm}
			\\
			$M=5$&&$M=10$&\\	\multicolumn{6}{c}{(c) Focused spots}		
		\end{tabular}
		\end{tabular}
		\caption{\footnotesize{\bf Fitting  transmission matrix:} 
			We fit a few types of transmission matrices with multi-slice model. The top panel tested physically accurate transmission matrices simulated with the Monte-Carlo approach of ~\cite{Bar:2020} at two optical depths.  Lower panels used a transmission matrices measured in the lab through layers of parafilm and mouse brain.    (a)  The reduction in fitting error as a function of the number of layers. (b) The averaged delivered energy (correlation between captured and fitted matrices). (c) %\Marina{(Dror) the spot was computed not captured. Maybe we should add this to methods?}\Anat{added a sentance in the main text} 
			An example of a spot behind the tissue using the wavefront estimated by the layered model, with  different number of layers. (for the M.C. matrices we only show focusing at $\od=5$).}\label{fig:fitting-all}
	\end{center}
\end{figure*}
%	{\raisebox{0.90cm}{\rotatebox[origin=c]{90}{Main Camera }}}&


==> cvpr_sec_files_cr/fig_numerical_sim_comp_spct.tex <==
\begin{figure*}[t!]
	\begin{center}
		\begin{tabular}{@{}c@{~~}c@{~}c@{}}	
			\includegraphics[height=0.17\textwidth]{figs/fitting_curves/spctrums_hor.pdf}&
			\includegraphics[height=0.17\textwidth]{figs/fitting_curves/fitTM_sprNA_OD5.pdf}&
			%\includegraphics[height=0.19\textwidth]{figs/fitting_curves/fitTMbyNA_OD20.pdf}&
			\includegraphics[height=0.17\textwidth]{figs/fitting_curves/fitTM_sprNA_OD40.pdf}\\
{\footnotesize	(a) Spectra} &{\footnotesize(b) $\od=0.5$}&	{\footnotesize 	 (c) $\od=4$}
		\end{tabular}\vspace{-0.2cm}

		\caption{\footnotesize {\bf Numerical simulation:} We synthesize transmission matrices using a very dense multi-layer model, and test how well we can fit them with a sparser set of layers. We compare two types of volumes, whose spectra are illustrated in (a). The first one has a random spectrum sampled from a uniform distribution, and the second  corresponds to a forward scattering spectrum with more content at the low frequencies.
			 We plot the square root of the fitting error as a function of the number of layers. As predicted in claim \ref{claim:quad-decay}, with a uniform spectrum this decays linearly with the number of layers until we pass the Nyquist limit. The error with the more realistic forward scattering spectrum decays much faster, but analytic characterization is harder.
			 We  compute the layers using a naive filtering of the ground truth as well as using gradient descent optimization. The naive filtering provides good results at low optical depths, as illustrated in (b), but fails at higher $\od$s as illustrated in (c).	}\label{fig:comp_spct}

	\end{center}\vspace{-0.2cm}
\end{figure*}


==> cvpr_sec_files_cr/fig_numerical_sim_varysup.tex <==
\begin{figure}[t!]
	\begin{center}
		\begin{tabular}{@{}c@{~}cc@{}}	
%			\includegraphics[height=0.19\textwidth]{figs/layer_support/layeres_support1.pdf}&
%	        \includegraphics[height=0.19\textwidth]{figs/layer_support/layeres_support2.pdf}&
%		    \includegraphics[height=0.19\textwidth]{figs/layer_support/layeres_support3.pdf}&
			\includegraphics[height=0.2\textwidth]{figs/fitting_curves/fitTMspr_varysup_zmax16_OD51.pdf}&
			%\includegraphics[height=0.19\textwidth]{figs/fitting_curves/fitTMbyNA_OD20.pdf}&
			\includegraphics[height=0.2\textwidth]{figs/fitting_curves/fitTMspr_varysup_zmax32_OD100.pdf}\\
	{{(a) $\smpthick=16\mu m$}}&{{(b) $\smpthick=32\mu m$}}
		\end{tabular}\vspace{-0.2cm}
		\caption{\footnotesize {\bf Layer support:} We plot the fitting error as a function of the number of layers for  volumes at two thicknesses. We evaluate fitting while varying the range $\prng$ covered by the transmission matrix.   Smaller supports can be fitted with fewer layers, since the local distribution of illumination angles is smaller, resulting in a lower range of axial frequencies.}\label{fig:numerical_sim}
	\end{center}\vspace{-0.2cm}
\end{figure}

